Common Failure Modes of Subcluster-based Sampling in Dirichlet Process Gaussian Mixture Models -- and a Deep-learning Solution

The Dirichlet Process Gaussian Mixture Model (DPGMM) is often used to cluster data when the number of clusters is unknown. One main DPGMM inference paradigm relies on sampling. Here we consider a known state-of-art sampler (proposed by Chang and Fisher III (2013) and improved by Dinari et al. (2019)), analyze its failure modes, and show how to improve it, often drastically. Concretely, in that sampler, whenever a new cluster is formed it is augmented with two subclusters whose labels are initialized at random. Upon their evolution, the subclusters serve to propose a split of the parent cluster. We show that the random initialization is often problematic and hurts the otherwise-effective sampler. Specifically, we demonstrate that this initialization tends to lead to poor split proposals and/or too many iterations before a desired split is accepted. This slows convergence and can damage the clustering. As a remedy, we propose two drop-in-replacement options for the subcluster-initialization subroutine. The first is an intuitive heuristic while the second is based on deep learning. We show that the proposed approach yields better splits, which in turn translate to substantial improvements in performance, results, and stability.

==> figures/2_cluster_random_init.tex <==
% \begin{figure}[t]%[h!]
%     \centering
%     % [1\linewidth]
%     {\includegraphics[width=0.8\linewidth,trim=0 1cm 0 0.5cm, clip, scale=0.4]
%     % {\includegraphics[scale=0.2]
%     {Figures/two_clusters.pdf}} 
    
%     \subcaptionbox{A single cluster (blue) that needs to be split.}
%     \label{fig:two_clusters:original}
    
%     % [1\linewidth]
%     {\includegraphics[width=0.8\linewidth,trim=0 1cm 0 0.5cm, clip, scale=0.4]
%     % {\includegraphics[scale=0.2]
%     {Figures/two_clusters_rand_init.pdf}}
    
%     \subcaptionbox{A random initialization of the labels (shown in 2 colors)}
%     \label{fig:two_clusters:random}
        
%     \caption{Random initialization ~\cite{Chang:NIPS:2013:ParallelSamplerDP}
%     yields 2 almost-identical Gaussians (visualized
%     by 2 almost-identical ellipses, in orange and blue). At this state, the proposed 
%     split will be rejected with a very high probability (\EQN\eqref{eqn:HastingRatioSplit}).
%     It will take at least several iterations before the 2-component GMM will imply 
%      a split that is likely to be accepted. }
%     \label{fig:two_clusters_init}
% \end{figure}
\begin{figure}[t]
\centering
%   \includegraphics[width=8cm,height=5cm]{Figures/random_split.png}%
    \subcaptionbox{A single cluster (blue) that needs to be split  \label{fig:two_clusters:original}}
    {\includegraphics[scale=0.5]{Figures/two_clusters.pdf}} 
    
    \subcaptionbox{A single cluster (blue) that needs to be split  \label{fig:two_clusters:random}}
    {\includegraphics[scale=0.5]{Figures/two_clusters_rand_init.pdf}} 
    % \caption{Random initialization ~\cite{Chang:NIPS:2013:ParallelSamplerDP} yields 2 almost-identical Gaussians (visualized by 2 almost-identical ellipses, in orange and blue). At this state, the proposed     split will be rejected with a very high probability (\EQN\eqref{eqn:HastingRatioSplit}). It will take at least several iterations before the 2-component GMM will imply a split that is likely to be accepted. }
\caption{Random Split Example 
\label{fig.two_clusters_init}}
\end{figure}



==> figures/__latexindent_temp.tex <==
\begin{figure}[h!]
    % \centering
        
      % \subcaptionbox{
        % A single cluster (blue) that needs to be split
        % \label{fig:clusters_random_init.original}}
      % [.95\linewidth]{\includegraphics[width=0.9\linewidth]{../figures/two_clusters.pdf}}\\
      % \subcaptionbox{
        %  A random initialization of the labels (shown in 2 colors)
        
        % \label{fig:clusters_random_init.random}
  [.95\linewidth]{\includegraphics[width=0.9\linewidth]{../figures/two_clusters_rand_init.pdf}}
  \caption[Random Initialization Example]{Random Initialization \cite{Chang:NIPS:2013:ParallelSamplerDP} yields 2 almost-identical Gaussians (visualized by 2 almost-identical ellipses, in orange and blue). At this state, the proposed split will be rejected with a very high probability (\EQN\eqref{eqn:HastingRatioSplit}). It will take at least several iterations before the 2-component GMM will imply a split that is likely to be accepted. }
\label{fig.clusters_random_init.random}
\end{figure}




==> figures/data_samples_copy.tex <==
\begin{figure}[t!]
\centering
  % \subcaptionbox{Easy Data Samples \label{fig:data_samples:easy}}
  % {\includegraphics[width=0.9\linewidth]{../figures/data_samples_easy.pdf}} 
  
  % \subcaptionbox{Medium Data Samples \label{fig:data_samples:medium}}
  % {\includegraphics[width=0.9\linewidth]{../figures/data_samples_med.pdf}}
  
  % \subcaptionbox{Hard Data Samples \label{fig:data_samples:hard}}
  % {\includegraphics[width=0.9\linewidth]{../figures/data_samples_hard.pdf}}
  
\includegraphics[width=0.98\linewidth]{../figures/data_samples_all.pdf}

\captionsetup{justification=justified, singlelinecheck=false}
\caption[Examples of Generated Training Data]{Examples of generated training data. Each panel represents a single training example; \ie, a cluster that needs to be split into two, according to the (ground-truth) colors. First row: ``easy'' data, middle row: ``medium-difficult'' data, last row: ``hard'' data.}
\label{fig:data_samples}
\end{figure} 


==> figures/fig_bad_prop.tex <==
\begin{figure}[h!]
\centering
  \subcaptionbox{The state before the first accepted split (iteration 16), using random initializations.
  \label{fig:theirs:iter16}}
  {\includegraphics[width=0.75\linewidth]{../figures/k=30_random_inter_16.png}}  \\
  % \hspace{0.05\linewidth} 
  % {\includegraphics[width=0.48\linewidth,trim=0 1cm 0 0.5cm clip]{../figures/k=30_random_inter_16.png}}  
  \subcaptionbox{The state before the first accepted split (iteration 4), using SplitNet initializations.
  \label{fig:ours:iter3}}
  {\includegraphics[width=0.75\linewidth]{../figures/k=30_splitnet_inter_4.png}}
  % {\includegraphics[width=0.48\linewidth,trim=0 1cm 0 0.5cm, clip]{Figures/k=30_splitnet_inter_4.png}}
   \captionsetup{justification=justified, singlelinecheck=false}
\caption{Intermediate stages of the example from \autoref{fig:intro}.
\label{fig:their16_vs_ours4}}
\end{figure}  


==> figures/log_HR_hist.tex <==
\begin{figure}[h!]%[h!]
\centering
%   [1\linewidth]
%   {\includegraphics[width=0.80\linewidth,trim=0 1cm 0 0.5cm clip]
  \subcaptionbox{
  Log HR Histogram on Easy Data
  \label{fig:loghr_hist:easy}}
  [0.4\linewidth]{\includegraphics[scale=0.4]{Figures/logHRhist_easy.png}} %
  \subcaptionbox
  {Log HR Histogram on Hard Data
  \label{fig:loghr_hist:hard}}
  [0.4\linewidth] {\includegraphics[scale=0.4]{Figures/logHRhist_hard.png}}
\caption[Log Hastings' Ratio Histograms on Training Datasets]{Log Hastings' Ratio Histograms on Training Datasets. It can be noticed that on the hard data, the model is able to propose better splits than $K$-means, as reflected by the density that is almost identical to the ground-truth one, whereas the $K$-means density is shifted towards lower values.}
\label{fig:loghr_hist}
\end{figure}  


%   \label{fig:data_samples:easy}

==> figures/result_2D_k40.tex <==
\begin{figure}[h!]
  \centering
  
  \subcaptionbox{
    Inferred $K$ vs. Iterations
    \label{fig:res:2d_k40:k}}
  [.24\linewidth]{\includegraphics[width=0.24\textwidth]{../figures/qual/D2_K40/fig_k.png}}
  \subcaptionbox{
     Log-Posterior vs. Iterations
    \label{fig:res:2d_k40:ll}}
  [.24\linewidth]{\includegraphics[width=0.24\textwidth]{../figures/qual/D2_K40/fig_ll.png}}
  \subcaptionbox{
    NMI vs. Iterations
    \label{fig:res:2d_k40:nmi}}
  [.24\linewidth]{\includegraphics[width=0.24\textwidth]{../figures/qual/D2_K40/fig_nmi.png}}
  \subcaptionbox{
    ARI vs. Iterations
    \label{fig:res:2d_k40:ari}}
  [.24\linewidth]{\includegraphics[width=0.24\textwidth]{../figures/qual/D2_K40/fig_ari.png}}
  
  \subcaptionbox{
    Ground Truth Labels
    \label{fig:res:2d_k40:gt_data}}
  [.24\linewidth]{\includegraphics[width=0.24\textwidth]{../figures/qual/D2_K40/data_Ground-Truth.png}}
  \subcaptionbox{
    Predictions with Random Init.
    \label{fig:res:2d_k40:pred_random}}
  [.24\linewidth]{\includegraphics[width=0.24\textwidth]{../figures/qual/D2_K40/data_Random.png}}
  \subcaptionbox{
    Predictions with $k$-means Init.
    \label{fig:res:2d_k40:pred_kmeans}}
  [.24\linewidth]{\includegraphics[width=0.24\textwidth]{../figures/qual/D2_K40/data_K-means.png}}
  \subcaptionbox{
    Predictions with SplitNet Init.
    \label{fig:res:2d_k40:pred_splitnet}}
  [.24\linewidth]{\includegraphics[width=0.24\textwidth]{../figures/qual/D2_K40/data_SplitNet.png}}
    
\caption[Split Types Comparison Results on 2D Data with K=40]{Comparison on 2D Data with K=40}
\label{fig:res:2d_k40}
\end{figure}

==> figures/split_stages_qual.tex <==
\begin{figure}[H]
    \centering
      \subcaptionbox{
        Random init.: the state before the first accepted split (iteration 5).
        \label{fig:qual_split_stages.random.pre}}
      [.48\linewidth]{\includegraphics[scale=0.1]{Figures/k=3_random_iter_5_pre.png}}
      \subcaptionbox{
         Random init.: the state after the first accepted split.
        \label{fig:qual_split_stages.random.post}}
      [.48\linewidth]{\includegraphics[scale=0.1]{Figures/k=3_random_iter_6_post.png}}
      
      
      \subcaptionbox{
        SplitNet init.: the state before the first accepted split (iteration 1).
        \label{fig:qual_split_stages.splitnet.pre}}
      [.48\linewidth]{\includegraphics[scale=0.1]{Figures/k=3_splitnet_iter_1_pre.png}}
      \subcaptionbox{
        SplitNet init.: the state after the first accepted split.
        \label{fig:qual_split_stages.splitnet.post}}
      [.48\linewidth]{\includegraphics[scale=0.1]{Figures/k=3_splitnet_iter_4_post.png}}


\caption[Random and SplitNet initializations]{Random and SplitNet initializations: with SplitNet, subclusters tend to converge faster. }
\label{fig.qual_split_stages}
\end{figure}


==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\RD}{\ensuremath{\RR^D}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}


\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern2pt}\sim\cr\noalign{\kern-2pt}}}}}


\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  

\definecolor{brown}{RGB}{165,42,42}
\newcommand{\BROWN}[1]{{{\color{brown}{#1}}}}



\newcommand{\FREIFELD}[1]{\textbf{\MAGENTA{[FREIFELD says: #1]}}}
% Make your own

\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}
\newcommand{\REPLACE}[2]{\RED{REPLACE:} \BLUE{#1} \RED{WITH:} \BLUE{#2}}



% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}
\bmdefine\bepsilon{\epsilon}


\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bsigma{\sigma}
\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbb{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


 \newcommand{\DP}{\mathrm{DP}}
 \newcommand{\DIR}{\mathrm{Dir}}


==> paper/__latexindent_temp.tex <==
\section{INTRODUCTION}\label{Sec:Intro}

This is the intro.
One of the best-performing BNP inference algorithms is the Dirichlet Process Gaussian Mixture Model (DPGMM) sampler by \cite{Chang:NIPS:2013:ParallelSamplerDP}, which was recently extended to a vastly-distributed and fast version by \cite{dinari2019distributed}. This sampler works in a split-merge framework, in which clusters splits and merges are proposed during inference to find the appropriate $K$ - the number of clusters of the data. These splits occur by randomly partitioning each existing cluster into two subclusters. More often than not, it is sufficient for the algorithm to converge and still provide the best results compared with other algorithms. 


Yet, we observe that under some conditions, namely, when the dataset is densely packed with partially overlapping clusters, the randomly proposed splits are mostly rejected. In the best-case scenario, this could lead to a "merely" inefficient, slow convergence. Beyond that, however, the sampler might get stuck in a poor local minimum and fail to converge to the proper clustering results. An example of such case, can be seen in \autoref{fig:intro:theirs}.

\subimport{./figs/}{fig_intro}

By identifying that the splits mechanism plays a crucial role in the sampler's performance, we set out to investigate methods to improve it. First, we consider a simple yet effective split mechanism that is based on $K$-means. Secondly, we propose and design a deep-learning-based model to "learn to split" data. We call it "SplitNet" and develop the architecture, data, and training procedures so that the model can propose the (close to) optimal splits, especially in the modes of failure that we've identified.


In the experimental study, we evaluate and compare the baseline sampler against the proposed ``smart splits``' and additional comparable DPGMM algorithms and test them on a comprehensive suite of synthetics simulations and real datasets. We show that the SplitNet based sampler outperforms the other methods in inference time and various clustering evaluation metrics.


\textbf{Our key contributions are:}
\begin{enumerate}
    \item We characterize and identify the failure modes of the sampler from \cite{Chang:NIPS:2013:ParallelSamplerDP}.
    \item We propose two "smart splits" methods which improve the DPGMM sampler from \cite{Chang:NIPS:2013:ParallelSamplerDP}, and in particular, we propose "SplitNet" - a data-driven deep learning framework for learning to split data.
\end{enumerate}


==> tables/tab_10D_K100.tex <==


\begin{table*}[h]
\centering
\caption{Results on Synthetic 10D Data with K=100}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}          & {NMI}                 & {ARI}                 & {Time [sec]}           \\ \midrule
    $K$-means			& - 						& 0.776	($\pm$ 0.006) 	& 0.491	($\pm$ 0.024)	& 34.83	($\pm$ 2.55) \\
    EM-GMM			& - 						& 0.945	($\pm$ 0.008) 	& 0.803	($\pm$ 0.050)	& 43.75	($\pm$ 8.47) \\ \midrule
    SK-DPGMM 			& 13.40	    ($\pm$ 4.42)	& 0.984	($\pm$ 0.002) 	& 0.986	($\pm$ 0.002)	& 250.95 ($\pm$ 57.97) \\
    moVB			& 75.30	    ($\pm$ 3.05)	& 0.702	($\pm$ 0.043) 	& 0.285	($\pm$ 0.084)	& 145.15 ($\pm$ 21.01) \\
    SubC-Random	& 3.90		($\pm$ 2.13)	& 0.993	($\pm$ 0.001) 	& 0.995	($\pm$ 0.001)	& \textbf{26.85	($\pm$ 2.52)} \\ 
    SubC-$K$-means	& 3.90		($\pm$ 1.72)	& 0.993	($\pm$ 0.001) 	& 0.994	($\pm$ 0.001)	& 32.35	($\pm$ 5.77) \\
    \textbf{SubC-SplitNet}	& \textbf{3.80		($\pm$ 2.15)}	& \textbf{0.994	($\pm$ 0.001) }	&\textbf{ 0.995	($\pm$ 0.001})	& 32.56	($\pm$ 4.94) \\
    \bottomrule
    \end{tabular}
\label{tab:10D_K100}
\end{table*}

==> tables/tab_10D_K200.tex <==


\begin{table*}[h!]
\centering
\caption{Results on Synthetic 10D Data with K=200}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}          & {NMI}                 & {ARI}                 & {Time [sec]}           \\ \midrule
    $K$-means			& -                     	& 0.858	($\pm$ 0.011)	& 0.579	($\pm$ 0.036)	& 118.17	($\pm$ 9.38) \\
    EM-GMM			& -                     	& 0.958	($\pm$ 0.006)	& 0.810	($\pm$ 0.043)	& 178.35	($\pm$ 22.19) \\ \midrule
    SK-DPGMM 			& 26.80 	($\pm$ 8.17)	& 0.995	($\pm$ 0.001)	& 0.996	($\pm$ 0.001)	& 892.99	($\pm$ 158.23) \\
    moVB			& 174.50    ($\pm$ 4.17)	& 0.600	($\pm$ 0.038)	& 0.107	($\pm$ 0.031)	& 393.97	($\pm$ 73.78) \\
    SubC-Random	& 23.10 	($\pm$ 61.83)	& 0.899	($\pm$ 0.316)	& 0.899	($\pm$ 0.316)	& 208.85	($\pm$ 71.18) \\
    SubC-$K$-means	& 22.90 	($\pm$ 61.90)	& 0.899	($\pm$ 0.316)	& 0.899	($\pm$ 0.316)	& 205.27	($\pm$ 74.82) \\
    \textbf{SubC-SplitNet}	&\textbf{ 3.30  	($\pm$ 2.00)}	& \textbf{0.999	($\pm$ 0.000)}	& \textbf{0.999	($\pm$ 0.000)}	& 250.70	($\pm$ 25.50) \\
    \bottomrule
    \end{tabular}
\label{tab:10D_K200}
\end{table*}

==> tables/tab_2D_K10.tex <==


\begin{table*}[t!]
\centering
\caption{Results on Synthetic 2D Data with K=10}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}      & {NMI}                 & {ARI}                 & {Time [sec]}           \\ \midrule
    $K$-means		    & -                 & 0.80	($\pm$ 0.09)	& 0.71	($\pm$ 0.15)	& 0.8	 ($\pm$ 0.2) \\ 
    EM-GMM			    & -                 & 0.84	($\pm$ 0.09)	& 0.75	($\pm$ 0.14)	& 0.4	 ($\pm$ 0.1) \\ \midrule
    SK-DPGMM 		    & 2.4	($\pm$ 1.5) 	& 0.81	($\pm$ 0.07)	& 0.75	($\pm$ 0.12)	& 371.5	($\pm$ 175.8) \\ 
    moVB			      & 0.1	($\pm$ 0.7) 	& 0.89	($\pm$ 0.07)	& 0.89	($\pm$ 0.08)	& 38.2  ($\pm$ 11.2) \\ 
    SubC-Random	    & 3.1	($\pm$ 2.1) 	& 0.83	($\pm$ 0.13)	& 0.77	($\pm$ 0.18)	& 2.9	 ($\pm$ 0.4) \\ 
    SubC-$K$-means	& 2.0	($\pm$ 1.4) 	& 0.88	($\pm$ 0.08)	& 0.85	($\pm$ 0.12)	& 3.0	 ($\pm$ 0.4) \\ 
    SubC-SplitNet	  & 1.6	($\pm$ 0.9) 	& 0.88	($\pm$ 0.06)	& 0.86	($\pm$ 0.09)	& 3.6	 ($\pm$ 0.4) \\ 
    \bottomrule
    \end{tabular}
\label{tab:2D_K10}
\end{table*}



% k-means			10.0	0.0		0.80	0.09	0.71	0.15	0.8		0.2
% EM-GMM			10.0	0.0		0.84	0.09	0.75	0.14	0.4		0.1
% DPGMM (SKlearn'	7.6		1.5		0.81	0.07	0.75	0.12	371.5	175.8
% moVB			9.9		0.7		0.89	0.07	0.89	0.08	38.2	11.2
% SubC-1-Random	6.9		2.1		0.83	0.13	0.77	0.18	2.9		0.4
% SubC-2-K-means	8.0		1.4		0.88	0.08	0.85	0.12	3.0		0.4
% SubC-3-SplitNet	8.4		0.9		0.88	0.06	0.86	0.09	3.6		0.4


==> tables/tab_2D_K20.tex <==


\begin{table*}[h!]
\centering
\caption{Results on Synthetic 2D Data with K=20}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}        & {NMI}                 & {ARI}                 & {Time [sec]}           \\ \midrule
    $K$-means		    & -					 		          & 0.86	($\pm$ 0.03)	& 0.73	($\pm$ 0.09)	& 1.1 	($\pm$ 0.1) \\
    EM-GMM			    & -					 		          & 0.87	($\pm$ 0.02)	& 0.75	($\pm$ 0.09)	& 0.5 	($\pm$ 0.1) \\ \midrule
    SK-DPGMM 		    & 8.6	    ($\pm$ 2.2)	    & 0.79	($\pm$ 0.04)	& 0.65	($\pm$ 0.10)	& 384.2 ($\pm$ 161.0) \\
    moVB			      & 4.2	    ($\pm$ 1.9)	    & 0.89	($\pm$ 0.04)	& 0.82	($\pm$ 0.13)	& 56.4  ($\pm$ 16.1) \\
    SubC-Random	    & 9.3	    ($\pm$ 3.5)	    & 0.83	($\pm$ 0.10)	& 0.69	($\pm$ 0.20)	& 3.4 	($\pm$ 0.7) \\
    SubC-$K$-means	& 7.6	    ($\pm$ 1.4)	    & 0.88	($\pm$ 0.04)	& 0.77	($\pm$ 0.13)	& 3.5 	($\pm$ 0.3) \\
    SubC-SplitNet	  & 8.5	    ($\pm$ 2.9)	    & 0.85	($\pm$ 0.10)	& 0.74	($\pm$ 0.18)	& 4.3 	($\pm$ 0.9) \\

    \bottomrule
    \end{tabular}
\label{tab:2D_K20}
\end{table*}
  
    
% k-means			      20.0	0.0		0.86	0.03	0.73	0.09	1.1		0.1
% EM-GMM			      20.0	0.0		0.87	0.02	0.75	0.09	0.5		0.1
% DPGMM 			      8.6	  2.2		0.79	0.04	0.65	0.10	384.2	161.0
% moVB			        4.2 	1.9		0.89	0.04	0.82	0.13	56.4	16.1
% SubC-1-Random	    9.3 	3.5		0.83	0.10	0.69	0.20	3.4		0.7
% SubC-2-K-means	  7.6 	1.4		0.88	0.04	0.77	0.13	3.5		0.3
% SubC-3-SplitNet	  8.5 	2.9		0.85	0.10	0.74	0.18	4.3		0.9


==> tables/tab_2D_K40.tex <==


\begin{table*}[h!]
\centering
\caption{Results on Synthetic 2D Data with K=40}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}          & {NMI}                 & {ARI}                 & {Time [sec]}           \\ \midrule
    $K$-means		    & -					                & 0.88	($\pm$ 0.02)	& 0.71	($\pm$ 0.07)	& 1.7 	($\pm$ 0.2) \\
    EM-GMM			    & -					                & 0.90	($\pm$ 0.03)	& 0.75	($\pm$ 0.08)	& 1.3 	($\pm$ 0.4) \\ \midrule
    SK-DPGMM 		    & 24.3	    ($\pm$ 1.7)	    & 0.75	($\pm$ 0.02)	& 0.49	($\pm$ 0.07)	& 622.6 ($\pm$ 72.3) \\
    moVB			      & 21.1	    ($\pm$ 4.8)	    & 0.84	($\pm$ 0.05)	& 0.59	($\pm$ 0.14)	& 76.7  ($\pm$ 26.2) \\
    SubC-Random	    & 30.0	    ($\pm$ 3.4)	    & 0.69	($\pm$ 0.13)	& 0.34	($\pm$ 0.15)	& 2.6 	($\pm$ 0.2) \\
    SubC-$K$-means	& 22.9	    ($\pm$ 7.2)	    & 0.81	($\pm$ 0.13)	& 0.57	($\pm$ 0.25)	& 3.7 	($\pm$ 0.9) \\
    SubC-SplitNet	  & 19.1      ($\pm$ 4.0)	    & 0.87	($\pm$ 0.03)	& 0.69	($\pm$ 0.10)	& 5.5 	($\pm$ 1.0) \\

    \bottomrule
    \end{tabular}
\label{tab:2D_K40}
\end{table*}



% k-means			    40.0	0.0		0.88	0.02	0.71	0.07	1.7		0.2
% EM-GMM			    40.0	0.0		0.90	0.03	0.75	0.08	1.3		0.4
% DPGMM 			    15.7	1.7		0.75	0.02	0.49	0.07	622.6	72.3
% moVB			      19.9	4.8		0.84	0.05	0.59	0.14	76.7	26.2
% SubC-1-Random	  10.0	3.4		0.69	0.13	0.34	0.15	2.6		0.2
% SubC-2-K-means	17.1	7.2		0.81	0.13	0.57	0.25	3.7		0.9
% SubC-3-SplitNet	20.9	4.0		0.87	0.03	0.69	0.10	5.5		1.0


==> tables/tab_3D_K20.tex <==


\begin{table*}[h]
\centering
\caption{Results on Synthetic 3D Data with K=20}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}              & {NMI}                     & {ARI}                     & {Time [sec]}           \\ \midrule
    $K$-means		& -								& 0.89	($\pm$ 0.03)		& 0.77	($\pm$ 0.09)		& 1.8	($\pm$ 0.1)  \\
    EM-GMM			& -								& 0.92	($\pm$ 0.02)		& 0.83	($\pm$ 0.07)		& 1.4	($\pm$ 0.6)  \\ \midrule
    SK-DPGMM 		& 0.5		($\pm$ 3.5)		    & 0.93	($\pm$ 0.02)		& 0.91	($\pm$ 0.04)		& 831.9	($\pm$ 358.4)  \\
    moVB			& 3.6	    ($\pm$ 2.2)		    & 0.94	($\pm$ 0.03)		& 0.90	($\pm$ 0.08)		& 64.8	($\pm$ 16.6)  \\
    SubC-Random	    & 0.9	    ($\pm$ 0.8)		    & 0.97	($\pm$ 0.01)		& 0.96	($\pm$ 0.02)		& 14.1	($\pm$ 0.6)  \\
    SubC-$K$-means	& 1.9	    ($\pm$ 2.0)		    & 0.96	($\pm$ 0.02)		& 0.95	($\pm$ 0.03)		& 13.3	($\pm$ 1.5)  \\
    SubC-SplitNet	& 1.2		($\pm$ 1.2)		    & 0.97	($\pm$ 0.01)		& 0.96	($\pm$ 0.02)		& 15.2	($\pm$ 1.0)  \\
    \bottomrule
    \end{tabular}
\label{tab:3D_K20}
\end{table*}


% k-means			20.0	0.0	    0.89	0.03	0.77	0.09	1.8		0.1
% EM-GMM			20.0	0.0	    0.92	0.02	0.83	0.07	1.4		0.6
% DPGMM 			0.5 	3.5	    0.93	0.02	0.91	0.04	831.9	358.4
% moVB			3.6 	2.2	    0.94	0.03	0.90	0.08	64.8	16.6
% SubC-1-Random	0.9 	0.8	    0.97	0.01	0.96	0.02	14.1	0.6
% SubC-2-K-means	1.9 	2.0	    0.96	0.02	0.95	0.03	13.3	1.5
% SubC-3-SplitNet	1.2 	1.2	    0.97	0.01	0.96	0.02	15.2	1.0


==> tables/tab_3D_K40.tex <==


\begin{table*}[h]
\centering
\caption{Results on Synthetic 3D Data with K=40}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}              & {NMI}                     & {ARI}                     & {Time [sec]}           \\ \midrule
    $K$-means		& -								& 0.88	($\pm$ 0.02)		& 0.70	($\pm$ 0.06)		& 3.6	($\pm$ 0.5)  \\
    EM-GMM			& -								& 0.92	($\pm$ 0.02)		& 0.81	($\pm$ 0.08)		& 4.1	($\pm$ 1.6)  \\ \midrule
    SK-DPGMM 		& 5.8		($\pm$ 3.1)		    & 0.86	($\pm$ 0.02)		& 0.77	($\pm$ 0.07)		& 1123.3($\pm$ 560.6)  \\
    moVB			& 20.6	    ($\pm$ 2.0)		    & 0.83	($\pm$ 0.03)		& 0.59	($\pm$ 0.10)		& 86.9	($\pm$ 16.8)  \\
    SubC-Random	    & 10.3	    ($\pm$ 6.1)		    & 0.92	($\pm$ 0.05)		& 0.86	($\pm$ 0.12)		& 15.7	($\pm$ 3.7)  \\
    SubC-$K$-means	& 9.9	    ($\pm$ 6.8)		    & 0.93	($\pm$ 0.04)		& 0.88	($\pm$ 0.08)		& 16.8	($\pm$ 3.4)  \\
    SubC-SplitNet	& 8.4		($\pm$ 4.0) 		& 0.94	($\pm$ 0.02)		& 0.90	($\pm$ 0.07)		& 22.2	($\pm$ 2.6)  \\
    \bottomrule
    \end{tabular}
\label{tab:3D_K40}
\end{table*}



% k-means			40.0	0.0	0.88	0.02	0.70	0.06	3.6		0.5
% EM-GMM			39.9	0.3	0.92	0.02	0.81	0.08	4.1		1.6
% DPGMM 			5.8 	3.1	0.86	0.02	0.77	0.07	1123.3	560.6
% moVB			20.6	2.0	0.83	0.03	0.59	0.10	86.9	16.8
% SubC-1-Random	10.3	6.1	0.92	0.05	0.86	0.12	15.7	3.7
% SubC-2-K-means	9.9	    6.8	0.93	0.04	0.88	0.08	16.8	3.4
% SubC-3-SplitNet	8.4	    4.0	0.94	0.02	0.90	0.07	22.2	2.6


==> tables/tab_3D_K80.tex <==


\begin{table*}[h]
\centering
\caption{Results on Synthetic 3D Data with K=80}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}          & {NMI}                 & {ARI}                 & {Time [sec]}           \\ \midrule
    $K$-means		&	- 						& 0.85	($\pm$ 0.02)	& 0.60	($\pm$ 0.05) 	& 7.3		($\pm$ 0.5) \\ 
    EM-GMM			&	- 						& 0.89	($\pm$ 0.01)	& 0.68	($\pm$ 0.05) 	& 9.2		($\pm$ 2.1) \\ \midrule
    SK-DPGMM		&	32.7	($\pm$ 3.7) 	& 0.79	($\pm$ 0.02)	& 0.57	($\pm$ 0.08) 	& 1545.5	($\pm$ 359.8) \\ 
    moVB			&	57.8	($\pm$ 2.8) 	& 0.73	($\pm$ 0.02)	& 0.37	($\pm$ 0.05) 	& 114.1	    ($\pm$ 23.0) \\ 
    SubC-Random	    &	62.0	($\pm$ 12.1) 	& 0.60	($\pm$ 0.25)	& 0.27	($\pm$ 0.25) 	& 9.8		($\pm$ 2.8) \\ 
    SubC-$K$-means	&	61.0	($\pm$ 11.3) 	& 0.66	($\pm$ 0.17)	& 0.30	($\pm$ 0.27) 	& 11.5		($\pm$ 4.5) \\ 
    SubC-SplitNet	&	44.5	($\pm$ 12.2) 	& 0.83	($\pm$ 0.08)	& 0.60	($\pm$ 0.21) 	& 22.8		($\pm$ 6.3) \\ 

    \bottomrule
    \end{tabular}
\label{tab:3D_K80}
\end{table*}


% k-means			80.0	0.0		0.85	0.02	0.60	0.05	7.3		0.5
% EM-GMM			80.0	0.0		0.89	0.01	0.68	0.05	9.2		2.1
% DPGMM 			32.7	3.7		0.79	0.02	0.57	0.08	1545.5	359.8
% moVB			57.8	2.8		0.73	0.02	0.37	0.05	114.1	23.0
% SubC-1-Random	62.0	12.1	0.60	0.25	0.27	0.25	9.8		2.8
% SubC-2-K-means	61.0	11.3	0.66	0.17	0.30	0.27	11.5	4.5
% SubC-3-SplitNet	44.5	12.2	0.83	0.08	0.60	0.21	22.8	6.3

==> tables/tab_5D_K100.tex <==


\begin{table*}[h]
\centering
\caption{Results on Synthetic 5D Data with K=100}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}      & {NMI}                 & {ARI}                 & {Time [sec]}           \\ \midrule
    $K$-means		& -                  	& 0.816	($\pm$ 0.014)	& 0.532	($\pm$ 0.043)	& 23.05	 ($\pm$ 1.95) \\ 
    EM-GMM			& -                  	& 0.904	($\pm$ 0.014)	& 0.728	($\pm$ 0.053)	& 40.05	 ($\pm$ 11.49) \\ \midrule
    SK-DPGMM 		& \textbf{4.80}	($\pm$ 3.67) 	& 0.893	($\pm$ 0.006)	& 0.873	($\pm$ 0.018)	& 292.64 ($\pm$ 19.94) \\ 
    moVB			& 74.80	($\pm$ 1.81) 	& 0.725	($\pm$ 0.025)	& 0.400	($\pm$ 0.073)	& 135.96 ($\pm$ 11.85) \\ 
    SubC-Random	    & 88.40	($\pm$ 14.38) 	& 0.315	($\pm$ 0.354)	& 0.141	($\pm$ 0.234)	& \textbf{4.62	 ($\pm$ 1.84)} \\ 
    SubC-$K$-means	& 51.30	($\pm$ 29.98) 	& 0.712	($\pm$ 0.381)	& 0.626	($\pm$ 0.391)	& 11.80	 ($\pm$ 5.79) \\ 
    SubC-SplitNet	& 39.90	($\pm$ 9.43) 	& \textbf{0.903	($\pm$ 0.022)}	& \textbf{0.841	($\pm$ 0.075)}	& 13.84	 ($\pm$ 2.01) \\ 
    \bottomrule
    \end{tabular}
\label{tab:5D_K100}
\end{table*}

==> tables/tab_acceptance_ratio.tex <==
% \begin{table*}[t]
% \caption{Acceptance/Rejection of the Splits} \label{tab:acceptance}
%     \begin{center}\small
%         \begin{tabular}{lccc}
%         \textbf{Init.~Type}  &\textbf{Burnout} &\textbf{Accepted/Proposed}  &\textbf{\# of Clusters}\\
%         \hline %\\
%         \textbf{Random}         & 18 & 796/6115=0.13 &      8.94 \\
%         \textbf{Eigensplits}    & 18 & 895/3670=\textbf{0.24} &    \textbf{9.93}\\
%         \textbf{Random}         & 3  & 227/3222=0.07 &     3.25\\
%         \textbf{Eigensplits}    & 3 & 1071/5045=\textbf{0.21} &    \textbf{11.59}\\
%         \end{tabular}
%     \end{center}
% \end{table*}

==> tables/tab_cifar10.tex <==


\begin{table*}[h]
    \centering
    \caption{Results on CIFAR10 Dataset, with 20D after PCA}
    \small
        \begin{tabular}{@{}l cccc@{}}
        \toprule
        Algorithm       & {\textit{k}-MAE}          & {NMI}                 & {ARI}                 & {Time [sec]}       \\ \midrule
        $K$-means			& -                     	& 0.796	($\pm$ 0.000)	& 0.777	($\pm$ 0.000)	& 1.69	($\pm$ 0.59) \\
        EM-GMM			& -                     	& 0.719	($\pm$ 0.000)	& 0.598	($\pm$ 0.001)	& 5.11	($\pm$ 1.31) \\ \midrule
        SK-DPGMM 			& 10.000	($\pm$ 0.000)	& 0.712	($\pm$ 0.004)	& 0.582	($\pm$ 0.004)	& 23.72	($\pm$ 7.67) \\
        moVB			& 14.000	($\pm$ 0.000)	& 0.681	($\pm$ 0.000)	& 0.529	($\pm$ 0.000)	& 146.44 ($\pm$ 4.37) \\
        SubC-Random	& 1.300	    ($\pm$ 0.675)	& 0.675	($\pm$ 0.026)	& 0.550	($\pm$ 0.040)	& 6.37	($\pm$ 1.38) \\
        SubC-$K$-means	& \textbf{1.000		($\pm$ 0.816)}	& 0.719	($\pm$ 0.024)	& 0.611	($\pm$ 0.046)	& 6.81	($\pm$ 1.22) \\
        SubC-SplitNet	& 2.000	    ($\pm$ 0.000)	& \textbf{0.736	($\pm$ 0.000)}	&\textbf{ 0.640	($\pm$ 0.001)}	& 8.56	($\pm$ 1.69) \\
        \bottomrule
        \end{tabular}
    \label{tab:CIFAR10}
    \end{table*}

==> tables/tab_cifar20.tex <==


\begin{table*}[h]
    \centering
    \caption{Results on CIFAR20 Dataset, with 20D after PCA}
    \small
        \begin{tabular}{@{}l cccc@{}}
        \toprule
        Algorithm       & {\textit{k}-MAE}          & {NMI}                 & {ARI}                 & {Time [sec]}           \\ \midrule
        $K$-means			& -                     	& 0.487	($\pm$ 0.000)	& 0.329	($\pm$ 0.000)	& 3.86	($\pm$ 0.55) \\
        EM-GMM			& -                     	& 0.437	($\pm$ 0.003)	& 0.237	($\pm$ 0.004)	& 10.47	($\pm$ 2.62) \\ \midrule
        SK-DPGMM 			& 20.00	    ($\pm$ 0.00)	& 0.441	($\pm$ 0.004)	& 0.198	($\pm$ 0.003)	& 54.69	($\pm$ 8.68) \\
        moVB			& 2.00	    ($\pm$ 0.00)	& 0.412	($\pm$ 0.000)	& 0.192	($\pm$ 0.000)	& 129.51 ($\pm$ 4.06) \\
        SubC-Random	& \textbf{6.90	    ($\pm$ 1.85)}	& 0.434	($\pm$ 0.009)	& 0.246	($\pm$ 0.011)	& 14.45	($\pm$ 2.27) \\
        SubC-$K$-means	& 8.20	    ($\pm$ 1.47)	& \textbf{0.457	($\pm$ 0.005)}	&\textbf{ 0.276	($\pm$ 0.006)}	& 15.10	($\pm$ 1.96) \\
        SubC-SplitNet	& 8.50		($\pm$ 1.95)	& 0.455	($\pm$ 0.005)	& 0.273	($\pm$ 0.005)	& 19.01	($\pm$ 6.03) \\
        \bottomrule
        \end{tabular}
    \label{tab:CIFAR20}
    \end{table*}


==> tables/tab_fmnist.tex <==


\begin{table*}[h]
\centering
\caption{Results on FMNIST Dataset, with 20D after PCA}
\small
    \begin{tabular}{@{}l cccc@{}}
    \toprule
    Algorithm       & {\textit{k}-MAE}          & {NMI}                 & {ARI}                 & {Time [sec]}              \\ \midrule
    $K$-means			& -                     	& 0.509	($\pm$ 0.010)	& 0.353	($\pm$ 0.004)	& 2.04 	($\pm$ 0.52)   \\
    EM-GMM			& -                     	& 0.571	($\pm$ 0.015)	& 0.380	($\pm$ 0.011)	& 2.91 	($\pm$ 1.11)  \\ \midrule
    SK-DPGMM 			& 10.00	    ($\pm$ 0.00)	& 0.573	($\pm$ 0.004)	& 0.347	($\pm$ 0.006)	& 14.95 ($\pm$ 0.67) \\
    \textbf{moVB}			&\textbf{ 0.00	    ($\pm$ 0.00)}	& \textbf{0.584	($\pm$ 0.000)}	& \textbf{0.386	($\pm$ 0.000)}	& 45.22 ($\pm$ 0.46)  \\
    SubC-Random	& 1.40	    ($\pm$ 0.54)	& 0.556	($\pm$ 0.009)	& 0.360	($\pm$ 0.008)	& 5.33 	($\pm$ 0.54)  \\
    SubC-$K$-means	& 1.60	    ($\pm$ 0.89)	& 0.572	($\pm$ 0.004)	& 0.362	($\pm$ 0.007)	& 6.11 	($\pm$ 0.63)  \\
    SubC-SplitNet	& 1.20		($\pm$ 2.16)	& 0.577	($\pm$ 0.007)	& 0.376	($\pm$ 0.008)	& 5.34 	($\pm$ 0.82)  \\
    \bottomrule
    \end{tabular}
\label{tab:FMNIST}
\end{table*}


==> tables/tab_stl10.tex <==


\begin{table*}[h]
    \centering
    \caption{Results on STL10 Dataset, with 20D after PCA}
    \small
        \begin{tabular}{@{}l cccc@{}}
        \toprule
        Algorithm       & {\textit{k}-MAE}      & {NMI}                 & {ARI}                 & {Time [sec]}       \\ \midrule
        $K$-means			& -                    	& 0.702	($\pm$ 0.000)	& 0.665	($\pm$ 0.000)	& 0.57	($\pm$ 0.07) \\
        EM-GMM			& -                    	& 0.607	($\pm$ 0.001)	& 0.457	($\pm$ 0.003)	& 1.13	($\pm$ 0.09) \\ \midrule
        SK-DPGMM 			& 10.00	($\pm$ 0.00)	& 0.628	($\pm$ 0.001)	& 0.511	($\pm$ 0.008)	& 6.81	($\pm$ 0.15) \\
        moVB			& 10.00	($\pm$ 0.00)	& 0.621	($\pm$ 0.000)	& 0.504	($\pm$ 0.000)	& 65.82 ($\pm$ 1.01) \\
        SubC-Random	& 1.80	($\pm$ 1.09)	& 0.597	($\pm$ 0.032)	& 0.467	($\pm$ 0.053)	& 1.62	($\pm$ 0.30) \\
        SubC-$K$-means	& 1.20	($\pm$ 0.83)	& 0.634	($\pm$ 0.021)	& 0.522	($\pm$ 0.039)	& 1.91	($\pm$ 0.50) \\
        \textbf{SubC-SplitNet}	& \textbf{1.00	($\pm$ 0.00)}	&\textbf{ 0.667	($\pm$ 0.001)}	& \textbf{0.557	($\pm$ 0.001)}	& 2.18	($\pm$ 0.31) \\
        \bottomrule
        \end{tabular}
    \label{tab:STL10}
    \end{table*}

